SelfReplay: Adapting Self-Supervised Sensory Models via Adaptive Meta-Task Replay

Self-supervised learning has emerged as a method for utilizing massive unlabeled data for pre-training models, providing an effective feature extractor for various mobile sensing applications. However, when deployed to end-users, these models encounter significant domain shifts attributed to user diversity. We investigate the performance degradation that occurs when self-supervised models are fine-tuned in heterogeneous domains. To address the issue, we propose SelfReplay, a few-shot domain adaptation framework for personalizing self-supervised models. SelfReplay proposes self-supervised meta-learning for initial model pre-training, followed by a user-side model adaptation by replaying the self-supervision with user-specific data. This allows models to adjust their pre-trained representations to the user with only a few samples. Evaluation with four benchmarks demonstrates that SelfReplay outperforms existing baselines by an average F1-score of 8.8%p. Our on-device computational overhead analysis on a commodity off-the-shelf (COTS) smartphone shows that SelfReplay completes adaptation within an unobtrusive latency (in three minutes) with only a 9.54% memory consumption, demonstrating the computational efficiency of the proposed method.

==> archived/abstract.tex <==
Self-supervised learning has emerged as a method for utilizing massive unlabeled data for pre-training models, providing an effective feature extractor for various mobile sensing applications. However, when deployed to end-users, these models encounter significant domain shifts attributed to user diversity. We investigate the performance degradation that occurs when self-supervised models are fine-tuned in heterogeneous domains. To address the issue, we propose \proj{}, a few-shot domain adaptation framework for personalizing self-supervised models. \proj{} proposes self-supervised meta-learning for initial model pre-training, followed by a user-side model adaptation by replaying the self-supervision with user-specific data. This allows models to adjust their pre-trained representations to the user with only a few samples. Evaluation with four benchmarks demonstrates that \proj{} outperforms existing baselines by an average F1-score of 8.8\%p. Our on-device computational overhead analysis on a commodity off-the-shelf (COTS) smartphone shows that \proj{} completes adaptation within an unobtrusive latency (in three minutes) with only a 9.54\% memory consumption, demonstrating the computational efficiency of the proposed method.

==> archived/evaluation.tex <==
We implement \proj{} based on additional self-supervised learning methods, further showing its generalizability. We incorporate two other self-supervised learning approaches popular in HAR: CPC~\cite{haresamudram2023investigating} and Multi-Task Learning~\cite{saeed2019multi}. Note that we do not extend \proj{} to be built on DARLING and Set-SimCLR. DARLING mainly offers an intra-domain negative sampling method, a concept we already integrate within \proj{} but with a different approach, focusing on creating small tasks for meta-learning. As for Set-SimCLR, it requires the training of a separate set encoder, which requires an additional training component to \proj{}, deviating from our framework's design.

To implement the backbone networks corresponding to the self-supervised learning methods, we used 1D convolutional neural networks (CNN) followed by a projection head of a fully connected layer. Our network design, including the architectures and hyperparameters, aligns with established practices in the prior assessment study~\cite{haresamudram2022assessing}. Specifically for CPC, we utilized the latest state-of-the-art version designed for HAR~\cite{haresamudram2023investigating}. We conducted a grid search to optimize the hyperparameters for each baseline. For pre-training, we explored learning rates from \{1e-4, 5e-4, 1e-3, 5e-3\}, batch sizes from \{64, 128, 256\}, with specific values of \{1024, 2048, 4096\} for SimCLR-based methods, and weight decays from \{0, 1e-4\}. During fine-tuning, we used a fixed learning rate of $0.005$ for the linear evaluation protocol and a reduced learning rate of $0.001$ for end-to-end fine-tuning, which exhibited superior performance. We trained models with 100 epochs for pre-training and 20 epochs for fine-tuning using Adam optimizer. We utilized parameters within the same range as the baselines for learning rate and weight decay for meta-learning. We searched for the task-specific learning rate from \{1e-3, 5e-3, 1e-2\} and the inner iteration steps for pretext replay from \{10, 20, 30\}. We kept the number of domain-specific tasks fixed at eight and multi-conditioned tasks at four. The task size was set to 128 for our evaluation. Note that meta-learning requires larger epochs for convergence than conventional training as fewer parameter updates happen inside an epoch; we set 5K epochs for meta-learning training. We implemented the methods using PyTorch, and the training was performed on NVIDIA TITAN Xp GPUs.

In the case of CPC, pretext replay enhances the baseline without meta-learning, while using only meta-learning yields poor results. Yet, when pretext replay is applied to the meta-learned model, performance significantly increases, exceeding the improvement observed from the baseline. This suggests that the adaptation step with pretext replay generally aids in learning meaningful features, and our meta-learning significantly amplifies this effect.

For Multi-Task Learning, pretext replay results in performance degradation in the baseline, while meta-learning improves it. Unlike SimCLR or CPC, the impact of pretext replay on the meta-learned model is minimal. Pretext replay slightly improves performance in HHAR and PAMAP2 while even slightly decreasing performance in DSA and ICHAR. This indicates that user-specific adaptation does not provide substantial benefits in the case of Multi-Task Learning. Importantly, meta-learning prevents pretext replay from significantly decreasing performance due to overfitting.

% \begin{figure*}
% % \setlength{\belowcaptionskip}{-8pt}
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/umap.pdf}
%     \caption{\jh{Should change the our system name in the Figure}2D UMAP visualizations of embeddings from CPC pre-trained models. Embeddings are color-coded by class.}% Results of before and after applying \proj{}'s pretext replay are shown.}
%     \label{fig:umap}
% \end{figure*}

% Figure~\ref{fig:umap} visualizes the effectiveness of pretext replay when combined with meta-learning, on a domain of ICHAR. We plot 2D UMAP visualizations~\cite{mcinnes2018umap} of embeddings from CPC pre-trained models, color-coded by class. Both CPC baseline and \proj{} before pretext replay lack distinct class-based clustering. It suggests that the models pre-trained out-of-domain fail to grasp meaningful features in the target domain. Meanwhile, \proj{} after pretext replay creates well-defined clusters aligned with class boundaries, demonstrating that pretext replay significantly enhances the model's ability to capture meaningful features within the target domain.

% In summary, our self-supervised meta-learning effectively supports pretext replay, enhancing target-domain performance by training the model to learn general features that can be rapidly refined into domain-specific features. Another finding is that the level of improvement varies depending on the self-supervised learning method. This observation leads us to hypothesize that self-supervised learning methods are differently affected by domain shifts, which we analyze further in the following section (Section~\ref{sec:domain_shift_effect}).

==> archived/introduction.tex <==
The integration of deep learning into mobile sensing has broadened the scope of ubiquitous applications, such as contactless authentication~\cite{wang2021ear, liu2022recent}, sign language translation~\cite{hou2019signspeaker, park2021enabling}, and mobile health applications~\cite{zhang2019pdmove, song2020spirosonic}. Nevertheless, a major challenge in mobile sensing is the scarcity of labeled data, which is often expensive to acquire. As a breakthrough, self-supervised learning~\cite{haresamudram2022assessing} has been explored for its ability to train models with unlabeled data and transfer knowledge to downstream tasks. Self-supervised learning methods, such as Contrastive Predictive Coding~(CPC)~\cite{haresamudram2021contrastive, haresamudram2023investigating}, similarity-based contrastive learning~(SimCLR)~\cite{tang2020exploring}, and Multi-Task Learning~\cite{saeed2019multi}, have been showing their effectiveness in sensory applications without needing explicit labels.

% The integration of deep learning into mobile sensing has broadened the scope of applications, such as contactless authentication~\cite{wang2021ear}, sign language translation~\cite{hou2019signspeaker}, and health applications~\cite{song2020spirosonic, li2023neuralgait}. To meet the growing demands for the applications, a paradigm of pre-training models with extensive data and fine-tuning them for various downstream tasks has emerged~\cite{zhuang2020comprehensive}. In particular, self-supervised learning~\cite{haresamudram2022assessing}  has been actively explored recently for training models with unlabeled data and transferring knowledge to downstream tasks. Self-supervised learning methods, such as Contrastive Predictive Coding~(CPC)~\cite{haresamudram2023investigating}, similarity-based contrastive learning~(SimCLR)~\cite{chen2020simple}, and Multi-Task Learning~\cite{doersch2017multi}, have been showing the their effectiveness in sensory applications~\cite{haresamudram2021contrastive, haresamudram2023investigating, tang2020exploring, saeed2019multi}. %Specifically, we target a scenario where individuals fine-tune the pre-trained models to align them with their own data.% their specific needs.

%A challenge arises in transitioning the pre-trained model to the end-user's fine-tuning.
A challenge arises when fine-tuning is performed by an end-user showing heterogeneity from the pre-training data. In mobile sensing, data collected in distinct environments varies significantly across individual users, devices, and settings (e.g., position and sampling rate)~\cite{ustev2013user}. Thus, the end-user data might have heterogeneous characteristics from those used for pre-training. 
%Thus, the data used for pre-training might have heterogeneous characteristics from those observed by end-users. 
This gap results in \textit{domain shift}, where models trained in one domain underperform when applied to another~\cite{stisen2015smart}. To illustrate this challenge within the self-supervised learning setting, we conducted an empirical analysis using CPC pre-trained models~\cite{haresamudram2023investigating} (experimental details in \S\ref{sec:domain_shift_effect}). In Fig.~\ref{fig:motivation_study}, the results show CPC is useful in downstream tasks when models are pre-trained in the same domain as the target domain (in-domain). However, there is a substantial decline in performance when models are pre-trained with different domains from the target domain (out-of-domain). This result emphasizes the challenges of deploying self-supervised models to diverse mobile sensing environments. %Based on the observation, we delve into the domain shift problem stemming from the self-supervised pre-trained models.
%Although fine-tuning was performed in domain, the results show a substantial decline in performance when pre-training occurred out of domain. 

\begin{figure}
% \setlength{\belowcaptionskip}{-6pt}
    \centering
    % \includegraphics[width=0.99\columnwidth]{figures/motivation_study_user.pdf}
    \includegraphics[width=\columnwidth]{figures/preliminary.pdf}
    \caption{\rev{Efficacy of CPC~\cite{haresamudram2023investigating} pre-trained models on ICHAR~\cite{gong2019metasense} dataset, comparing F1-scores between in-domain and out-of-domain pre-training scenarios. Ten participants with different devices are shown as domains. Domain shifts deteriorate the performance of self-supervised models in heterogeneous environments.}}
    \label{fig:motivation_study}
\end{figure}

Training a domain-specific model with data from the end user could be a straightforward solution, but this is infeasible considering the efforts and cost of gathering enough data from an individual user. To address the challenge, existing research encompasses domain generalization methods~\cite{qian2021latent, qin2022domain, lu2022semantic}, which strive to train domain-invariant features, or domain adaptation techniques~\cite{chang2020systematic, gong2019metasense, zhou2020xhar, wang2018stratified} that leverage a small portion of target domain data to achieve domain-specific performance. However, they primarily rely on labeled data for training, making them difficult to be applied to self-supervised learning which utilizes only unlabeled data for pre-training. %Additionally, our focus is on the domain shift between pre-training and fine-tuning stages, which was not investigated in the existing literature. %In our scenario, testing and fine-tuning occur in the same target domain. However, the domain gap originating from the pre-training phase can still pose significant challenges.
%differs from existing methods in perceiving domain shift. While most existing methods focus on the gap between training and testing domains, we focus 

To mitigate the issue, we propose \proj{} as a few-shot domain adaptation framework to refine the self-supervised model into a personalized model specific to the end user. Inspired by the capability of meta-learning to ``learn to learn'' from few-shot data, we adapt the concept to our unsupervised pre-training setting. We introduce \textit{self-supervised meta-learning} for pre-training, which enables the model to ``learn to self-supervise'' with only a few data. This results in the model being adaptable to the learning task of self-supervised pre-training, \ie{} \textit{pretext task}. Next, we synergistically harness the adaptability by involving \textit{pretext replay} as a pivotal domain adaptation step. The end-user engages in adapting the pre-trained model by replaying the pretext task using its own few-shot data. This process effectively aligns the model to the representation reflecting the end user's domain property with very few data. %, thereby mitigating the impact of domain shifts.
It is noteworthy that our framework is designed to be agnostic to the self-supervision algorithm, and thus, it can be integrated into existing self-supervision methods. Fig.~\ref{fig:intro_overview} outlines a comparative overview of \proj{}'s operation against the standard self-supervised learning.

\begin{figure}
% \setlength{\belowcaptionskip}{-6pt}
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/method_summary.pdf}
    \caption{A high-level comparison between the standard self-supervised learning (left) and \proj{}(right).}
    \label{fig:intro_overview}
\end{figure}

% % original
% To address the domain shift challenges, we propose \proj{}, a novel framework that facilitates few-shot domain adaptation for self-supervised learning. First, \proj{} pre-trains models via \textit{self-supervised meta-learning}. This technique integrates self-supervised learning into meta-learning optimization, allowing for rapid adaptation to tasks with very few data. Second, \proj{} further refines the pre-trained model on the end-user side via a process named \textit{pretext replay}. Specifically, in the \textit{pretext replay} step, we adapt the pre-trained model for the target domain with the same pretext task but with a small amount of target domain data. This adapted model is then used for fine-tuning towards a specific downstream task. The rationale behind pretext replay is to align the model to the target domain as if it was pre-trained with target domain data, thereby mitigating the impact of domain shifts. In addition, our meta-learning component is a key enabler of effective pretext replay with very few samples from the target domain.

%We find that this additional adapting step is useful in improving transferability towards fine-tuning.
%Pre-training is followed by a few-shot domain adaptation to refine the pre-trained model on the end-user side. This is achieved by training the model via the pretext task used for pre-training, using few-shot target-domain data. This \textit{pretext replay} step is reinforced by the pre-trained model's adaptability to the pretext task, simulated during the self-supervised meta-learning. 
% This adapted representation is then used for fine-tuning towards the downstream tasks, tailored to user applications.

% Our intuition behind employing pretext replay is straightforward: inadequately pre-trained models lead to suboptimal performance after fine-tuning. As models pre-trained out-of-domain function inadequately on the target side (Figure~\ref{fig:motivation_study}), we align the model as if to be pre-trained on the target domain, by additionally training the same pretext task using the target domain data. Note that target-side end-users lack data, which may lead to overfitting. To facilitate this adaptation in data-scarce environments, meta-learning is adopted as our core component.

% Our approach is grounded in the observation (\S\ref{sec:domain_shift_effect}) that a model pre-trained within the same domain shows better transferability towards fine-tuning. %For instance, a model pre-trained on motion data from a younger user group may struggle to extract relevant features from elderly groups, potentially misinterpreting characteristics like decreased activity level, while performing well in the younger group. 
% Our pretext replay is designed to adjust the model to learn end-user-specific features within the same pretext task, and meta-learning is employed to facilitate few-shot adaptation considering the data scarcity.

% We evaluate \proj{} under domain shifts between the unlabeled pre-training and few-shot fine-tuning data. %On four real-world datasets with domain shifts, ICHAR~\cite{gong2019metasense}, HHAR~\cite{stisen2015smart}, PAMAP2~\cite{reiss2012introducing}, and DSA~\cite{altun2010comparative}, 
For evaluation, we used four Human Activity Recognition datasets~\cite{gong2019metasense, stisen2015smart, reiss2012introducing, altun2010comparative} that are representative datasets used for evaluating the performance under domain shifts. Our experiments demonstrate the superior performance of \proj{} to %three state-of-the-art self-supervised learning baselines~\cite{oord2018representation, chen2020simple, saeed2019multi} and two 
domain generalization and adaptation baselines~\cite{zhang2022towards, lee2023self}, exhibiting a high F1-score that shows an $8.83\%$p improvement on average. 
%. \proj{} exhibits a high F1-score that shows an $8.83\%$p improvement on average compared to the baselines. 
To further assess the practical viability of executing fine-tuning with domain adaptation on mobile devices, we measure the computational overhead of \proj{} on an off-the-shelf smartphone. Our evaluation reveals that the adaptation step with pretext replay can be completed within three minutes, indicating marginal user-side computational overhead while achieving improved performance.

We summarize our main contributions as follows:

\begin{itemize}[left=1em, topsep=0pt, partopsep=0pt]

\item We investigate the domain shift problem arising when self-supervised models are deployed to diverse users for fine-tuning. %in widely used self-supervised learning on mobile sensing applications. 
%\item We explore a practical domain shift scenario, where domain shift occurs between the unlabeled pre-training and labeled fine-tuning data. 
Our research reveals that even after fine-tuning the pre-trained model with target domain data, the domain shift from the pre-training data can lead to significant performance degradation.

\item We introduce \proj{}, a few-shot domain adaptation framework that can be integrated into existing self-supervised learning methods. 
%a self-supervised learning method-agnostic framework designed for few-shot domain adaptation of models pre-trained without labels. 
\proj{} incorporates self-supervised meta-learning for the pre-training and target-side pretext replay, enabling the adaptation of pre-trained representations to the target domain using only a few target samples.

\item We perform rigorous evaluations using four mobile sensing datasets %~\cite{gong2019metasense, stisen2015smart, reiss2012introducing, altun2010comparative} 
with diverse domain characteristics. We compare \proj{} against %three self-supervised learning baselines and two 
domain generalization/adaptation baselines%~\cite{zhang2022towards, lee2023self}, %, oord2018representation, chen2020simple, saeed2019multi}. Our results show
, that shows \proj{} achieves an average F1-score improvement of $8.83\%$p.

\item We assess the computational overhead of deploying \proj{} on real-world mobile applications and demonstrate that the one-time target-side adaptation can be executed within three minutes %by utilizing 3.4 CPU cores 
by consuming a mere $9.54\%$ of the device's memory on a COTS smartphone. %, making it practical for real-world mobile applications.
\end{itemize} 
% \begin{figure}
%     \vspace{0.8cm}
%     \centering
%     \includegraphics[width=0.4\columnwidth]{figures/intro.pdf}
%     \caption{\hj{Just the concept drawing. Will be replaced with a pretty icons and drawings.}}
%     \label{fig:problem_scenario}
% \end{figure}

==> archived/methodology.tex <==
%%%%% OVERVIEW %%%%%

We present \proj{} as a framework designed to effectively tune a deployed self-supervised model into a personalized model on an end user's device. %Our approach aims to address the domain shift between the data used for self-supervised pre-training and the end user's data. %To achieve this, \proj{} modifies the typical pipeline of pre-training and fine-tuning self-supervised models (Fig.~\ref{}).
% utilizes the end user's data, facilitating additional self-supervised training on the representation model. However, considering the practical scenario in which end users have access to only a few samples, the scarcity of training samples could lead to overfitting. To address the challenge, we introduce a novel approach designed to enable the models to adapt effortlessly to the few-shot self-supervised learning. We propose self-supervised meta-learning, optimizing models via meta-learning during the unsupervised pre-training. Note that \proj{} is designed to be agnostic to both model architecture and the self-supervised learning method used for pre-training.
% We address the challenge by introducing a novel approach to pre-train models via self-supervised meta-learning. This method is designed to enable the models to adapt effortlessly to the few-shot self-supervised learning of the end user. Note that \proj{} is designed to be agnostic to both model architecture and the self-supervised learning method used for pre-training.
Fig.~\ref{fig:project_overview} shows \proj{} unfolds through two core stages: (1) pre-training models via \textit{self-supervised meta-learning} and (2) adapting pre-trained models via \textit{pretext replay}. The process begins with a model provider, utilizing a large amount of unlabeled data to train the model with a self-supervised objective optimized via meta-learning. This method is designed to enable the models to adapt effortlessly to the few-shot self-supervised learning of the end user. Once trained, these models are deployed to the edge devices of end users. Each user then engages in a domain adaptation process, replaying the learning task of the self-supervised pre-training (\ie{} pretext task) with the user's own few-shot data. This results in the model achieving a personalized representation, akin to having been pre-trained with the same user's data. The tuned models are subsequently fine-tuned again with few-shot labeled data, this time for downstream tasks, similar to the original self-supervised learning. Further details about these processes will be elaborated in the following sections.

% % original
% We aim to address the domain shift problem when pre-trained models are fine-tuned in heterogeneous target domains. To achieve our goal, we present \proj{}, a few-shot domain adaptation method to refine pre-trained representations to align with the target domain. Figure~\ref{fig:project_overview} shows \proj{} unfolds through two core stages. First, we perform \textit{self-supervised learning via meta-learning} for pre-training models without labels. \proj{} defines meta-learning tasks composed of only a few domain-specific data, optimizing for self-supervised learning objective (\ie{} pretext task). This approach results in a pre-trained model that is highly adaptable to the pretext task with few-shot examples from a single domain. Next, target-side few-shot fine-tuning is performed. We split this fine-tuning into two adaptation stages: domain adaptation using \textit{pretext replay} and adaptation to the downstream task objective. Our domain adaptation refines the model while replaying the same pretext task used for pre-training but with target domain data in this stage. Thanks to the adaptability achieved through meta-learning, the model is effectively refined as a pre-trained model tailored for the target domain. Afterward, we fine-tune the domain-adapted model for the end-user application, optimizing it for the downstream task objective with labels.

%Our goal is to optimize the performance of pre-train models when they are fine-tuned for a distinct target domain. 
% We present \proj{}, a domain adaptation approach to refine pre-trained representations for effective application in heterogeneous target domains. As depicted in Figure~\ref{fig:project_overview}, \proj{} unfolds through two core stages. First, model providers perform self-supervised pre-training via meta-learning. \proj{} defines meta-learning tasks composed of only a few data divided by domains to be optimized with self-supervised objectives. This approach generates a highly adaptable model to the pretext task based on limited data from a single domain. Next, we fine-tune the pre-trained model using few-shot examples collected from end-users. We divide the fine-tuning step into two adaptation stages: %(1) first, \proj{} fine-tunes the model using end-users' data while replaying the same pretext task used for pre-training and (2) then we further update the model using labeled data based on downstream task objective.
% the first \textit{ADAPT} towards the target domain via \textit{pretext replay} and the second \textit{ADAPT} towards the downstream task. To tailor the pre-trained model to their specific domain, \proj{} fine-tunes the model using end-users' data while replaying the same pretext task used for pre-training. This step outputs an adapted user-specific model, which is finally fine-tuned for downstream tasks.

%This adaptation makes the model face the simulated training environment of meta-learning, effectively fitting it to the target domain using only a few examples. The domain-adapted model trains the downstream tasks specific to the application.

%%%%% PROBLEM FORMULATION %%%%%

% % original
% We target a setup where (1) pre-training is performed using large, unlabeled data and (2) fine-tuning using very few labeled data. This setup reflects the difficulties of acquiring privacy-sensitive label information from the model provider side and collecting enough training data from the end-user side. We assume model providers have access to the domain information indicating distinct user or device characteristics, considering the practicality of acquiring those data as metadata, even in anonymized form.

% We denote the pre-training dataset with $N^{\text{pt}}$ samples as $S^{\text{pt}}=\left\{(x_i, d_i) \,|\, i=1...N^{\text{pt}}\right\}$ where $x_i$ represents sensor data and $d_i$ represents the domain information (\eg{} anonymized user or device). The source domain $D^s$ is composed of the set of domain labels, \ie{} $d_i \in D^s$. %for all domain labels.
% % The superset of $d_i$ comprises the source domain $D^s$, \ie{} $D^s=\cup_{i=1}^{N^{\text{pt}}}d_i$. 
% The fine-tuning dataset with $N^{\text{ft}}$ samples is defined as $S^{\text{ft}}=\left\{(x_i, y_i) \,|\, i=1...N^{\text{ft}}\right\}$, where label $y_i$ of downstream task is available with sensor data $x_i$. Data $x_i$ in $S^{\text{ft}}$ originates from a single target domain $D^t$, which is distinct from $D^s$, \ie{} $D^t \cap D^s = 
%  \emptyset$. The fine-tuned model is tested in the same target domain $D^t$.

Our target scenario is the same as typical self-supervised learning, where a model is pre-trained through self-supervision with unlabeled data, followed by fine-tuning on a target task (in our case, this is an end user's edge device) using very few labeled data. This approach is designed to reflect two key challenges: the difficulty of obtaining costly annotations for pre-training, and the constraints faced by end users in gathering enough data and executing large-scale training on resource-limited edge devices. We explore a setup where data for self-supervised pre-training originate from domains that are completely separate from that of the end user. We assume the availability of domain labels in the pre-training data. Domain labels involve the type of measurement device or anonymized user annotation, which are generally more accessible to acquire as metadata.

% \textbf{Notations.} We use $x$, $y$, and $d$ to indicate the sensory feature, label, and domain information (\eg{} anonymized user or device), respectively. We denote the unlabeled pre-training dataset with $N^{\text{pt}}$ samples as $S^{\text{pt}}=\left\{(x_i, d_i) \,|\, i=1...N^{\text{pt}}\right\}$. The set of $d_i$ in $S^{\text{pt}}$ composes the source domain, referred as $D^s$. The fine-tuning dataset with $N^{\text{ft}}$ samples is defined as $S^{\text{ft}}=\left\{(x_i, y_i) \,|\, i=1...N^{\text{ft}}\right\}$, where label $y_i$ is available. Data $x_i$ in $S^{\text{ft}}$ originates from a single target domain $D^t$, which is distinct from $D^s$, \ie{} $D^t \cap D^s = 
%  \emptyset$. The fine-tuned model is tested in the same target domain $D^t$.

%%%%% METASSL %%%%%
% \proj{} performs self-supervised learning to pre-train models. % via meta-learning. 
% As label information is not accessible in $S^{\text{pt}}$, parameter update with supervised objectives of the traditional meta-learning cannot be applied. Instead, we replace the supervised objectives of task-specific weight optimization with a pretext (\ie{} self-supervised) task that can be defined without labels. 
% Integrating self-supervised objectives into meta-learning is agnostic to the type of the pretext task. In this study, we focus on the three most widely-used self-supervised learning methods in mobile sensing: CPC~\cite{oord2018representation}, SimCLR~\cite{chen2020simple}, and Multi-Task Learning~\cite{saeed2019multi}.
% With the integration of self-supervised learning objectives, meta-learned models learn \textit{how to learn with the pretext task}. This implies its adaptability towards few-shot fine-tuning is not on the downstream task but on the pretext task. To fully utilize this adaptability, we perform a few-shot adaptation via the same pretext task in the following step. We detail this target-side \textit{pretext replay} in \S\ref{sec:pretext_replay}.

% % original
% Given the data scarcity from end-users, \proj{} employs meta-learning~\cite{andrychowicz2016learning} for pre-training for few-shot adaptation in the later stage. Our meta-learning implementation is based on Model-Agnostic Meta-Learning (MAML)~\cite{finn2017model}. We aim to identify the model parameters that effectively perform pretext tasks within new domains in minimal gradient steps. Our objective closely aligns with the core idea of training initial parameters for optimal performance on new tasks with minimal gradient updates. Furthermore, the model-agnostic nature of MAML ensures \proj{}'s adaptability to different types of self-supervised learning methods (\eg{} CPC, SimCLR, and Multi-Task Learning).%, expanding its utility across a wider spectrum of applications.

% %to facilitate applicability across various training objectives (\eg{} CPC, SimCLR, and Multi-Task Learning). In contrast to typical training, 
% In MAML, meta-learning composes a set of tasks (denoted as $\mathcal{T}$) that simulates few-shot learning and the corresponding evaluation. Using only a few examples, the model trains task-specific weights, $\theta_i$, within each task, $\mathcal{T}_i$. The dataset used for training the task-specific weights is denoted as a \textit{support set}, \ie{} $\mathcal{S}_i$. The trained task-specific weights are then evaluated on a distinct dataset named a \textit{query set}, \ie{} $\mathcal{Q}_i$. The evaluation results %for each task-specific weight 
% from each task are aggregated over all tasks and generate a loss value to optimize the actual model weights. Through this iteration, the model learns \textit{how to learn over few-shot samples} for higher performance by mimicking the few-shot adaptation within a task.

% We carefully design the meta-learning task $\mathcal{T}$ to facilitate domain-specific few-shot adaptation (stage~2 in Figure~\ref{fig:project_overview}). As we aim to adapt the model to %the environment of 
% a single target domain, we define each task to compose $\mathcal{S}_i$ and $\mathcal{Q}_i$ from a single domain by replicating the later adaptation. We call these composed tasks domain-specific tasks. %Besides, the pre-trained model should be able to adapt to diverse, unseen domains. 
% For each $\mathcal{T}_i$, a single domain is randomly selected from the source domain set $D^s$. 
% % Besides, for pre-training the model to learn adaptable weights towards diverse and unseen domains, we compose %the dataset of 
% % each task $\mathcal{T}_i$ by different, randomly selected domains. 
% We further mitigate the risk of overfitting to domains based solely on $D^s$ by leveraging multi-conditioned tasks~\cite{gong2019metasense}. The multi-conditioned tasks are formed by random samples selected regardless of the domain, thus working as new types of domains. With a small portion of randomly sampled tasks, we avoid the potential overfitting to the source-domain-specific features.  Algorithm~\ref{alg:task_generation} summarizes our task generation.

% % original
% Algorithm~\ref{alg:ssml} describes the parameter update conducted with self-supervised meta-learning. For each generated task, $\mathcal{T}_i$, we train task-specific weights $\theta_i$ with a task-specific learning rate, denoted as $\alpha$ (Line 4). The task-specific weights are then evaluated using the query set (Line 5), and the evaluated losses are aggregated over all tasks to update the model parameter $\theta$ (Line 7), where $\beta$ represents the meta-learning rate. For all optimizations, we define the parameterized function $f_\theta$ and the corresponding loss function $\mathcal{L}$ to align with the self-supervised pretext task. 

% For instance, if the pretext task is CPC, the loss function is designed to enhance distinguishability by encouraging the model to differentiate the true future embedding ($g_\theta({x_i^{t+j}})$) from other candidate embeddings ($g_\theta({x_i^l})$). This is achieved by comparing the similarity with the prediction from aggregated embedding before the time step ($f_\theta(x_i^{t})$). Denoting the parameterized encoder as $g_\theta$, predictor as $f_\theta$, and segmented data of $x_i$ at time step $t$ as $x_i^t$, we use the loss function defined as
% % enhance distinguishability by encouraging the model to differentiate the true future embedding from other candidate embeddings by comparing the similarity with the aggregated embedding before the time step. $f_\theata$, $g_\theata$, $h_\theata$ are parameterized functions for aggregator, encoder, and predictor

% % \begin{equation}
% % \mathcal{L}_{\text{CPC}} = -\log\left(\frac{e^{\text{sim}(\mathbf{z}_{t+j}, \mathbf{c_t})}}{e^{\text{sim}(\mathbf{z}_{t+j}, \mathbf{c_t})} + \sum_{k=1}^{K}e^{\text{sim}(\mathbf{z}_k, \mathbf{c_t})}}\right), \label{eq:cpc}
% % \end{equation}
% % \vspace{-2mm}
% \begin{equation}
% \mathcal{L}^{\text{CPC}}(\theta;S) = - \sum_{x_i\in S} \log\left(\frac{e^{\text{sim}(g_\theta(x_i^{t+j}), f_\theta(x_i^t))}}{e^{\text{sim}(g_\theta(x_i^{t+j}), f_\theta(x_i^{t}))} + \sum_{l\neq j}e^{\text{sim}(g_\theta(x_i^{t+l}), f_\theta(x_i^{t}))}}\right). \label{eq:cpc}
% \end{equation}
% % \begin{equation}
% % \mathcal{L}^{\text{CPC}}(\theta;S) = - \sum_{x_i\in S} \sum_{t=1}^{T} \sum_{j=1}^{J} \log\left(\frac{e^{\text{sim}(g_\theta(x_i^{t+j}), h_\theta(f_\theta(x_i^t)))}}{e^{\text{sim}(g_\theta(x_i^{t+j}), h_\theta(f_\theta(x_i^{t})))} + \sum_{l\neq j}e^{\text{sim}(g_\theta(x_i^{t+l}), h_\theta(f_\theta(x_i^{t})))}}\right), \label{eq:cpc}
% % \end{equation}

% For SimCLR, the loss function is set to minimize the similarity between the embeddings of two augmented views of the same data ($x'_i$ and $x''_i$) while ensuring dissimilarity with other data points ($x_k$). With the parameterized encoder $f_\theta$, the loss becomes
% % \begin{equation}
% % \mathcal{L}_{\text{SimCLR}} = -\log\left(\frac{e^{\text{sim}(\mathbf{z}_i, \mathbf{z}_j)}}{e^{\text{sim}(\mathbf{z}_i, \mathbf{z}_j)} + \sum_{k=1}^{K}e^{\text{sim}(\mathbf{z}_k, \mathbf{z}_j)}}\right),
% % \end{equation}
% % \vspace{-3mm}
% \begin{equation}
% \mathcal{L}^{\text{SimCLR}} (\theta; S) = - \sum_{x_i\in S} \log\left(\frac{e^{\text{sim}(f_\theta(x'_i), f_\theta(x''_i))}}{e^{\text{sim}(f_\theta(x'_i), f_\theta(x''_i))} + \sum_{k\neq i} e^{\text{sim}(f_\theta(x'_i), f_\theta(x_k))}}\right). \label{eq:simclr}
% \end{equation}

% Multi-Task Learning loss is assessed by comparing the probability %$h_\theta^t(f_\theta(x'_i))$ 
% $p_\theta^t(x'_i)$ of an internal prediction task $t$, which involves predicting whether an augmentation is applied to $x'_i$, to an automatically generated label $y_t$ indicating the occurrence of augmentation. Denoting $T$ as the set of prediction task and $p_\theta^t$ as the task-specific classifier composed of an encoder $f_\theta$ and task-specific prediction head $h_\theta^t$ of task $t$, \ie{} $p_\theta^t=h_\theta^t\circ f_\theta$, the loss becomes

% % \begin{equation}
% % \mathcal{L}_{\text{MTL}} = -\sum_{t \in T} \left[y_t \cdot \log(p_t) + (1 - y_t) \cdot \log(1 - p_t)\right], \label{eq:multi}
% % \end{equation}
% % \vspace{-3mm}
% % \begin{equation}
% % \mathcal{L}^{\text{MTL}} (\theta; S) = - \sum_{x_i\in S} \sum_{t \in T} \left[y_t \cdot \log(h_\theta^t(f_\theta(x'_i))) + (1 - y_t) \cdot \log(1 - h_\theta^t(f_\theta(x'_i)))\right]. \label{eq:multi}
% % \end{equation}
% \begin{equation}
% \mathcal{L}^{\text{MTL}} (\theta; S) = - \sum_{x_i\in S} \sum_{t \in T} \left[y_t \cdot \log(p_\theta^t(x'_i)) + (1 - y_t) \cdot \log(1 - p_\theta^t(x'_i)))\right]. \label{eq:multi}
% \end{equation}

% Based on the replaced optimization, our meta-learning procedure produces a model adaptive to a specific domain's data for the \textit{self-supervised pretext task}. This enhanced adaptability simplifies the subsequent design of the \textit{pretext replay} step, further facilitating domain adaptation to the target domain.

%%%%% REPLAYSSL %%%%%
We introduce \textit{pretext replay} as the core methodology for our few-shot domain adaptation. This adaptation involves refining the model using the same self-supervised learning objective (\ie{} pretext task) as in the pre-training step but with the end user’s data. This step serves as an additional training stage on the user's edge device, facilitating domain adaptation prior to the actual fine-tuning for the subsequent supervised downstream task (\textit{e.g.}, Human Activity Recognition).

Importantly, pretext replay demonstrates its effectiveness when coupled with self-supervised meta-learning. On the contrary, typical self-supervised models are prone to overfitting when exposed to few-shot training through pretext replay. Similarly, relying solely on self-supervised meta-learning without the subsequent pretext replay step does not yield optimal adaptability for supervised fine-tuning. We propose pretext replay as the unique key bridging the self-supervised pre-training and the subsequent supervised fine-tuning, enabled by the integration of meta-learning in self-supervised pre-training. This synergy between the self-supervised meta-learning and pretext replay is the core aspect of our approach, and its efficacy is validated in an ablation study detailed in \S\ref{sec:ablation}.

The model weights, $\theta$, are updated using the parameterized function and the corresponding loss $\mathcal{L}_\texttt{SSL}$, originating from the self-supervised meta-learning. Pretext replay uses the fine-tuning data set $S^\text{ft}$, without labels, and is performed in a few steps (e.g., 10) with a fixed learning rate, as formulated in the equation:
\begin{equation}
\theta \gets \theta-\alpha \nabla_{\theta} \mathcal{L}_\texttt{SSL}(\theta;S^\text{ft}) \text{.}
\end{equation}

After the adaptation, the model undergoes fine-tuning for the downstream task, which is similar to the normal self-supervised learning setup. $S^\text{ft}$ with the label information is employed to fine-tune $\theta$ towards the downstream task. We utilize the popular linear evaluation protocol~\cite{wu2018unsupervised} for fine-tuning, only training a simple classification head attached after the frozen encoder. The final model trained through this fine-tuning is used for the end-user application.

% % original
% After pre-training, \proj{} conducts domain adaptation with the target domain data, using the meta-learned pretext task (\eg{} CPC, SimCLR, or Multi-Task Learning) as the training objective. This process, represented as \textit{pretext replay}, functions as an additional pre-training step within the target domain. Its goal is to develop a domain-specific representation that can be effectively applied to the downstream tasks in the target domain. Our intuition behind pretext replay is straightforward: models pre-trained out-of-domain tend to yield sub-optimal performance for fine-tuning in the target domain. To address this issue, we align the model as if it were pre-trained on the target domain by additionally training the same pretext task using the target domain data. %Note that target-side end-users lack data, which may lead to ineffective training. We highlight that this pretext replay is enabled in data-scarce environments by meta-learning that trains adaptability toward the pretext task.
% % While pretext tasks in self-supervised learning requires a massive number of data to learn effective representations, our self-supervised meta-learning allows pretext replay to fast adapt to target domain with a limited number of samples.

% % Our intuition behind employing pretext replay is that inadequately pre-trained models lead to suboptimal performance after fine-tuning. As models pre-trained out-of-domain function inadequately on the target side, we align the model as if to be pre-trained on the target domain, by additionally training the same pretext task using the target domain data. Note that target-side end-users lack data, which may lead to overfitting. To facilitate this adaptation in data-scarce environments, meta-learning is adopted in the previous stage.

% % Our intuition behind this adaptation is based on our empirical observations (detailed in \S\ref{sec:domain_shift_effect}) indicating that pre-trained models from different domains often suffer a significant performance drop in downstream tasks, even after fine-tuning with the target domain data. Recognizing that a domain shift from the pre-training domain leads to this performance drop, our approach refines the pre-trained model, aligning it more closely with a model pre-trained on the target domain.

% Pretext replay uses few-shot samples from $S^{\text{ft}}$. While pretext tasks in self-supervised learning require massive data to learn effective representations, our self-supervised meta-learning allows pretext replay to adapt fast to the target domain with a limited number of samples. Combining self-supervised meta-learning with pretext replay makes \proj{} an effective solution for end-users with limited data.

% We update the pre-trained model weights $\theta$ by reusing the parameterized function and the corresponding loss $\mathcal{L}$ originated from the pretext task (\eg{} $\mathcal{L}^\text{CPC}$, $\mathcal{L}^\text{SimCLR}$, or $\mathcal{L}^\text{MTL}$). Here, the data used for the training is $S^\text{ft}$, but without labels. The adaptation is performed in a few steps (\eg{} 10), with a fixed learning rate. The parameter update is formulated as 
% %\vspace{-3mm}
% % \begin{equation}
% % \theta \gets \theta-\alpha \nabla_{\theta} \mathcal{L}(\theta;S^\text{PR}) \text{, where } S^\text{PR} = \{x_i \,|\, (x_i, y_i) \in S^{\text{ft}}, i=1...N^\text{ft}\} \text{.}
% % \end{equation}
% \begin{equation}
% \theta \gets \theta-\alpha \nabla_{\theta} \mathcal{L}_\texttt{SSL}(\theta;S^\text{ft}) \text{.}
% \end{equation}

% After the adaptation, the model is finally fine-tuned to the specific downstream task for the end-user application (\eg{} human activity recognition or gesture recognition). $S^\text{ft}$ with the label information is used for the fine-tuning of $\theta$ towards downstream tasks. We utilize the linear evaluation protocol~\cite{wu2018unsupervised} for fine-tuning, only training a simple classification head attached after the frozen encoder. The final model trained through this fine-tuning is used for the end-user application.

